Language-Guided Audio-Visual Source Separation via Trimodal Consistency

We propose a self-supervised approach for learning to perform audio source separation in videos based on natural language queries, using only unlabeled video and audio pairs as training data. A key challenge in this task is learning to associate the linguistic description of a sound-emitting object to its visual features and the corresponding components of the audio waveform, all without access to annotations during training. To overcome this challenge, we adapt off-the-shelf vision-language foundation models to provide pseudo-target supervision via two novel loss functions and encourage a stronger alignment between the audio, visual and natural language modalities. During inference, our approach can separate sounds given text, video and audio input, or given text and audio input alone. We demonstrate the effectiveness of our self-supervised approach on three audio-visual separation datasets, including MUSIC, SOLOS and AudioSet, where we outperform state-of-the-art strongly supervised approaches despite not using object detectors or text labels during training.

==> old_approach.tex <==
\section{Approach}

\begin{enumerate}
    \item After reading through Section 3 and thinking over the contributions, I think you should make the two new training losses the hero of the paper. My suggestion is to reorder the subsections as follows: (1) Section 3.3, (2) Section 3.2. You can put the current Section 3.1 into the current Section 3.2 (see comment below). The current Section 3.3 needs a lot more motivation/intuition, so this reordering will force you to write more to make it clear. 
    \item Section 3.1 primarily includes low-level model training details. I would create a "Training" paragraph in the current Section 3.2 and move most of the current Section 3.1 content there. 
\end{enumerate}

Given a set of unlabeled videos and their accompanying audios, our goal is to learn to separate audio sources based on multimodal queries in a self-supervised manner. To this end, we propose a novel \modelname approach that learns effective audio representations for audio-visual source separation as well as a strong alignment between the audio and natural language modalities. Our approach consists of an audio encoder that extracts latent representations from an input audio spectrogram and a decoder that predicts a real-valued ratio spectrogram mask that corresponds to a query. 

To facilitate the model to learn to separate audio sources based on video or natural language queries, our approach encourages it to learn a projection of the audio representations to the joint visual-semantic embedding space learned by large-scale pretrained vision-language foundation models. Our key insight is to use videos as the intermediary modality to learn a \emph{transitive} relationship between the audio and natural language modalities. Intuitively, this helps the model learn to separate audio components with language queries by training only on unlabeled videos. However, we observe in our initial experiments that using CLIP visual representations in SOTA audio-visual separation approaches results in learnt audio representations that do not have a strong transitive alignment with the natural language modality. We circumvent this by introducing the Kullback-Leibler (KL) divergence and cyclic consistency loss functions that encourages the audio encoder to learn a mapping that is well-aligned with both visual and natural language modalities. We begin by defining the problem formulation in Section~\ref{sec:problem_definition} before describing our \modelname in Section~\ref{sec:model_arch}. Finally, we present the novel KL divergence and cyclic consistency losses in Section~\ref{sec:alignment_losses}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/latent_concept_motivational_figure_v1.pdf}
    \caption{Extraction of latent concepts for pseudo-supervision. }
    \label{fig:latent_extraction}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/combined_model_figure_v2.pdf}
    \caption{Combined approach. }
    \label{fig:latent_extraction}
\end{figure*}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.5\textwidth]{Figures/model_figure.pdf}
%    \caption{In this work, we endeavor to determine the effectiveness of leveraging powerful pretrained image-and-text foundation models such CLIP and ALIGN for multimodal sound source separation in videos under the open-vocabulary setting. }
%    \label{fig:motiv}
%\end{figure}

\subsection{Problem formulation}\label{sec:problem_definition}
We define an audio mixture $A$ as a combination of multiple audio sources $A = \{a_1, \cdot\cdot\cdot, a_N \}$, where $N$ is the number of audio source components in the mixture. We assume that each potential audio source is emitted by an object, visible or otherwise. Consequently, we can formalize the audio mixture mathematically as $A = \sum_{i=1}^N a_i$, where $a_i$ is the linear audio waveform of the $i$-th source component. This allows us to also consider the presence of ambient sounds by treating them as originating from an unseen object in the video.

Consistent with state-of-the-art audio-visual separation approaches [], we adopt the 'mix-and-separate' self-supervised training strategy. Specifically, we select a pair of videos $V_1$ and $V_2$ and combine their corresponding audio components $A_1$ and $A_2$ to compute a mixed audio waveform $A = A_1 + A_2$. We apply Short-time Fourier transform (STFT) on the mixed waveform to compute its magnitude spectrogram $A^S$ and phase $A^{\text{phase}}$, which encodes how the magnitude of the waveform frequency change over time. Our learning algorithm uses only the magnitude spectrogram $A^S \in \mathbb{R} ^ {FxT}$, where F and T are the number of frequency bins and STFT frames, respectively.

Given the input audio spectrogram and any combination of natural language and video queries, the objective is to compute a real-valued ratio spectrogram mask $\hat{M}$ for the input mixed audio spectrogram that corresponds to the query. The predicted mask is applied to the mixed audio spectrogram using the Hadamard product to compute the final predicted spectrogram. Finally, we can apply inverse STFT on the predicted magnitude spectrogram with its phase value to reconstruct the predicted audio waveform. 

\subsection{\modelname}\label{sec:model_arch}
Our Video-Audio-Text Separation (VATS) model comprises an audio model as well as visual and language encoders. We use the pretrained CLIP model as our visual and language encoders to exploit its learnt visual-semantic alignment. Given a natural language query $L \in \mathbb{R}^{N_w}$ where $N_w$ is the number of words, we extract its representation $f_L \in \mathbb{R}^{1 \text{x} D}$ using the text encoder: $f^L = g_\phi^L(L)$, where $D$ is the dimension of CLIP joint visual-semantic space and $g_\phi^L(L)$ denotes its language encoding function that is parameterized by $\phi$. For a video consisting of $T_v$ frames $V = \{V_1, \cdot\cdot\cdot, V_{T_v} \}$, we extract a spatial grid of region representations $f^V \in \mathbb{R}^{T_v x H' x W' x D}$, where $H'$ and  $W'$ denote the downsampled height and width of the input video clip, respectively. We encode each frame separately:
\begin{equation}
    f^V_{t} = g_\theta^V(V_t), 
\end{equation}
where $g^V_\theta$ is CLIP visual encoding function that is parameterized by $\theta$.  We note that the language queries are only used during inference. 

Additionally, we adopt the U-Net \cite{ronneberger2015u} model, which has been demonstrated by prior work \cite{zhao2018sound} to be effective at audio source separation. The audio U-Net model comprises an encoder and decoder components. Given an input audio spectrogram $A^S$, the encoder component $\mathcal{E}$ passes it through a series of downsampling convolutional layers to output a set of bottleneck features $f^A \in \mathbb{R}^{H^A \text{x} W^A \text{x} D}$, where $H^A$ and $W^A$ are the height and width of the downsampled spectrogram, respectively. This operation is identical for language queries. We enforce that the audio U-Net encoder learns a mapping of its representations directly into CLIP visual-semantic embedding space so that it will be able to use both visual and language queries for audio separation. Given a visual representation $f^V$ as query , we tile the visual representation by the factor $H^A W^A$ and concatenate them with the audio bottleneck representations along the channel dimension: 
\begin{equation} \label{eq:tile_concat_op}
    f^{AV} = concat(f^A, tile(f^V)),
\end{equation}
where $f^{AV}$ has the dimensions $\mathbb{R}^{H^A \text{x} W^A \text{x} D}$. Finally, we pass the concatenated representations into the decoder component $\mathcal{D}$ consisting of a series of upsampling convolutional layers to generate a real-valued ratio mask $\hat{M} \in \mathbb{R}^{F \text{x} T}$ that can be multiplied with the input spectrogram via elementwise product. This operation is formulated mathematically as: $\hat{M} = \mathcal{D}(f^{AV})$.

In the mix-and-separate learning strategy, we generate pseudo-target ratio masks for training supervision. Given a pair of ground-truth audio spectrograms $A_1^S$ and $A_2^S$, we compute their ratio masks as follows:
\begin{equation}
    M_1 = \frac{A_1^S}{A_1^S + A_2^S} \quad\text{and}\quad 
    M_2 = \frac{A_2^S}{A_1^S + A_2^S}
\end{equation} 
We adopt the mask prediction loss \cite{zhao2018sound} to train the audio U-Net model for audio separation. Given the pair of predicted masks $\hat{M_1}$ and $\hat{M_2}$, we compute the mask prediction loss as:
\begin{equation}
    \mathcal{L}_{mask} = || \hat{M}_1 - M_1 ||_1 + || \hat{M}_2 - M_2 ||_1
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/sample_clip_attn_1.pdf}
    \caption{\textbf{CLIP text-visual attention heatmaps for different objects / instruments.}}
    \label{fig:motiv}
\end{figure}

\noindent \textbf{Multiple Instance Learning for video region mask prediction. } We explore two different granularity of audio source separation - \emph{video-level} and \emph{region-level}. In \emph{video-level} separation, we can compute a video-level representation by performing the maxpooling operation over the spatiotemporal grid of region features as follows: $f^V_{\text{video}} = \text{maxpool}\limits_{r \in T_v H'W'}(f^V_r)$. This can be fused with the audio bottleneck representations in Equation~\ref{eq:tile_concat_op}. 

While video-level source separation works well for videos with single object, prior work [] has demonstrated that object-level representations result in significantly improved performance in source separation for videos with multiple objects. In the absence of object detectors, we adopt a Multiple Instance Learning (MIL) framework, where all visual regions are treated as positive candidates. Specifically, given a spatiotemporal grid of region representations extracted from the visual encoder as defined in Section~\ref{sec:model_arch},  we predict a spectrogram mask $\hat{M}_{t,r}$ for the $r$-th region in the $t$-th frame. Finally, we compute an aggregated spectrogram mask for the entire video:
\begin{equation}
    \hat{M} = \frac{1}{T_v}\sum\limits_{t=1}^{T_v}\sum\limits_{r=1}^{H'W'}\hat{M}_{t,r}.
\end{equation}
Intuitively, this formulation encourages the model to learn to identify the salient regions with sounding objects for audio separation. We only enforce this constraint within frames and average the predicted masks over temporal dimension due to our reasoning that the same sounding object should have similar prediction masks across frames.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/cyclic_text_loss.pdf}
    \caption{\textbf{Cyclic loss with CLIP text representations in audio-visual source sound separation.}}
    \label{fig:motiv}
\end{figure}

While using videos as an intermediary modality sounds like a straightforward way to learn a \emph{transitive} alignment between the audio and natural language modalities, our initial experiments demonstrate SOTA audio-visual separation approaches do not generalize well to language queries despite using CLIP visual representations. Consequently, we introduce the Kullback–Leibler (KL) divergence $\mathcal{L}_{KL}$ and cyclic consistency $\mathcal{L}_{cons}$ losses to facilitate the audio U-Net learning audio representations that are well-aligned to both visual and natural language modalities, which we describe in the following section. The final objective function is computed as the sum of all three loss components:
\begin{equation*}
    \mathcal{L}_{final} = \lambda_1 \mathcal{L}_{mask} + \lambda_2 \mathcal{L}_{KL} + \lambda_3 \mathcal{L}_{cons}
\end{equation*}
where $\lambda_1$, $\lambda_2$ and $\lambda_3$ denote the weights for the mask prediction, KL divergence and cyclic consistency loss components, respectively.

\subsection{Aligning audio representations with visual and natural language concepts}\label{sec:alignment_losses}
As mentioned above, using CLIP visual representations in SOTA audio-visual separation approaches does not help them learn to separate audio sources with language queries. This suggests that simply learning an alignment between the audio and visual modalities does not preserve the \emph{transitive} relationship between the latter and natural language. More interestingly, these approaches also perform significantly worse with CLIP visual representations as compared to those of ImageNet-pretrained visual encoders []. We hypothesize that this is due to information about written words and their visual concepts being disentangled in CLIP visual embedding space \cite{Materzynska_2022_CVPR}. 

Materzynska \etal \cite{Materzynska_2022_CVPR} show that it is possible to disentangle the visual concepts by learning linear projection functions with supervision from the language representations of the object class labels. In the absence of object labels in the unlabeled videos, we adapt the pretrained CLIP model to extract a latent caption $V*$ for each video $V$ (Figure~\ref{fig:latent_extraction}). We begin by encoding the center frame of a video $V_{center}$ as: $f^V_{center} = g_\theta^V(V_{center})$. Then, we replace the token embeddings used for language queries with a learnable parameter $p$ and encode it using the language encoder: $V* = g_\phi^L(p)$. We optimize the weights of the learnable parameter $p$ by maximizing the cosine similarity between $f^V_{center}$ and $V*$:
\begin{equation}
    \max_{p} sim(\frac{f^V_{center}}{||f^V_{center}||_2}, \frac{V*}{||V*||_2}).
\end{equation}
Intuitively, a latent caption should embody the visual concepts present in its corresponding video. These latent captions are used for pseudo-text supervision in place of ground-truth object labels. We begin by extracting the audio representation of a predicted spectrogram $\hat{A}$ in Section~\ref{sec:model_arch}: $\hat{f}^A = \mathcal{E}(\hat{A})$ and averaging over the spatial regions.

\subsubsection{Attention KL divergence loss}\label{sec:kl_loss}
To learn a transitive alignment between the learnt audio and CLIP text representations via the intermediary visual modality, we enforce that the learnt audio representation of the predicted spectrogram is grounded correctly in the relevant spatiotemporal regions. Prior work [] have demonstrated that the CLIP model can be engineered to extract a segmentation map. Inspired by this, we use the latent concepts to provide pseudo-target attention maps. Specifically, for a given video $V$, we compute a probability distribution of similarity scores over the set of spatial region features with respect to its latent concept $V^*$:
\begin{equation}
    P_{Att}(VL) = softmax(f^V V^{*T})
\end{equation}
Next, we compute a similar distribution over the region features with respect to the encoded audio representation of the masked spectrogram:
\begin{equation}
    P_{Att}(AV) = softmax(f^V \hat{f}^A^T)
\end{equation}
We encourage the predicted audio representation to learn a similar mapping to that of the latent concept by minimizing the Kullback-Leibler (KL) divergence between the two attention distributions:
\begin{equation}
    \mathcal{L}_{KL}(P_{Att}(VL) || P_{Att}(AV)) = \mathbb{E}_{V \sim P_{AV}}[\log \frac{P_{Att}(VL)}{P_{Att}(AV)}]
\end{equation}

\subsubsection{Latent caption consistency loss}\label{sec:cons_loss}

Additionally, we further improve the alignment between the predicted audio representations and CLIP visual-semantic embedding space by encouraging them to be consistent with their latent captions. Intuitively, the audio sources that are well-separated by the visual cues should have a strong semantic relevance to the latent captions that describe the visual cues.
In lieu of the object labels, we maximize the similarity between the predicted audio representations and the latent concepts. Mathematically, we can formulate this as:
\begin{equation*}
    \mathcal{L}_{cons} =
-\sum_{i=1}^{n} \log (\frac{\exp(\hat{f}^A \cdot V^*)}{\hat{f}^A  \cdot V^* + \sum_{V^{*'}} \exp(\hat{f}^A  \cdot V^{*'})} )
\end{equation*}
where $V^{*'}$ is a negative latent caption that does not correspond to the predicted audio.
In theory, this is similar to the self-supervised multimodal learning objective of maximizing the similarity between the representations of an image and its corresponding caption as well as the dissimilarity of non-corresponding captions. We hypothesize that using a low weight for this loss component is likely to be more beneficial since some videos may contain similar sounding objects. In that case, maximizing the dissimilarity between the predicted audio and latent captions with similar sounding objects may make the effect of false negatives more pronounced. 

==> old_introduction.tex <==


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/motivational_figure_v13.pdf}
    \caption{In this work, we address the task of self-supervised audio source separation in unlabeled videos by extracting latent concepts from large-scale pretrained visual-and-language model.}
    \label{fig:latent_motiv}
\end{figure}

\section{Introduction v5}

\begin{enumerate}
    \item \textbf{BR:} add a paragraph at the beginning to motivate the importance of natural language and the overall task (and maybe point to/cite the success of other language-vision tasks). For example, natural language provides an intuitive and flexible interface for selecting sounds. You could also make the point that the co-occurrence of a sounding object and its depiction in video helps a model learn to identify and separate the sound from the background, and that we want to learn this co-occurrence from audio-video pairs without human supervision.
    \item \textbf{BR:} I think it would be good to articulate clearly the key challenge that this paper addresses: how to jointly localize sounding objects in both a video and an audio waveform, and to associate both with natural language, all in a self-supervised way. You can then point out that prior work learns to associate separated audio with bounding boxes detected for a set of fixed-vocabulary categories. Your approach and key contribution (and I think you can make this point stronger) leverages the recent success of vision-language foundation models (e.g., CLIP) for overcoming this challenge. You show how to incorporate CLIP into a prior mix-and-separate (Sound of Pixels) approach for source separation. Finally, you introduce two novel losses for self-supervised learning.
    \item \textbf{BP:} When you talk about what removing the bounding boxes would enable ("We believe that"), you could also bring up the fact that this restricts what categories of objects you can separate the sounds from (which you don't explicitly state, at least so far in my reading)
    \item \textbf{BP:} In the paragraph starting with "To the best of our knowledge" you make it seem like you are doing the same thing as prior work
    \item \textbf{BP:} You make some reference to the assumptions of prior work, but again, don't explicitly state them when you bring up the "mix and separate" part of the discussion.  It makes it hard for me to follow how you are doing something different
\end{enumerate}

Separating audio sources in videos or based on natural language queries is an inherently challenging problem since the input audio is usually a mixture of sounds from different objects and there is a lack of ground-truth source annotations. To ease the difficulty of this task, state-of-the-art multimodal source separation approaches often rely on strong supervision in the form of human-annotated captions [] and trained object detectors [] for audio-text and audio-visual separation, respectively. However, training object detectors to identify possible regions of interest (Figure~\ref{fig:latent_motiv} top) may not always be feasible due to insufficient bounding box annotations for objects in the long-tailed distribution. More importantly, this severely limits their capability to learn from an abundance of unlabeled data videos online. In contrast, we, as humans, have an innate ability to separate the mixed audio input into its individual components and attribute each one to a potential object, visible or otherwise, when we perceive the environment around them.

Inspired by this capability, we endeavor to address the above-mentioned limitations by learning to separate audio sources based on any combination of video and natural language queries without strong supervision, illustrated in Figure~\ref{fig:latent_motiv} (bottom). We believe that alleviating the need for human-annotated captions and bounding box supervision during training will open up the possibility for learning to perform multimodal audio source separation from the plethora of unlabeled videos online, allowing approaches to generalize well to a large variety of audio sources. Similar to how humans often leverage object sounds to understand their states and interactions with other objects, multimodal audio source separation is integral to improving machine perception of our environment. It has important implications in downstream applications including holistic video understanding [], embodied AI [] and bidirectional audio-to-video retrieval [].

To the best of our knowledge, we propose the first completely self-supervised approach for learning to separate audio source components with text and/or video queries from unlabeled videos without object labels or text captions at all. Due to a lack of ground-truth source annotations in videos, existing approaches often adopt the 'mix-and-separate' strategy where audios from multiple video clips are combined and the learning objective is to separate the audio components based on visual cues of the individual videos. Our approach adopts the same strategy but uses a Multiple Instance Learning (MIL) formulation to learn to perform source separation at the \emph{region} level without making assumptions on the presence of objects in the videos. The absence of text annotations in these videos raises the question of how our approach can learn to separate audio components with natural language queries despite not training with them. To this end, we adapt large-scale pretrained models to extract latent concepts and leverage them for pseudo-target supervision in the form of two novel loss functions. 

These loss formulations stem from our key intuition that a model has to learn a strong alignment between the visual, language and audio representations such that text and videos can be used interchangeably or in combination to perform source separation. To this end, we impose cyclic consistency losses where the spatiotemporal region features in the video are first used to separate the corresponding audio source before maximizing the similarity between the representation of the final predicted audio source and the latent concept in two different ways. Intuitively, this allows the model to identify regions with the most relevant visual concepts for source separation, facilitating its ability to learn from multi-source videos without prior knowledge of possible objects or their positions.

Despite not relying on trained object detectors, our proposed approach outperforms strongly-supervised state-of-the art-approaches by a significant margin across multiple datasets. More significantly, we demonstrate that our trained model can also separate sound sources based on natural language queries despite not having access to ground-truth object labels or using text representations during training. In summary, our contributions are listed as follows:
\begin{enumerate}
    \item To the best of our knowledge, we propose the first fully self-supervised approach to learn to separate audio source components with video and/or natural language queries from unlabeled videos.
    \item We introduce two novel loss functions that leverage latent concepts to learn a strong alignment between the audio, text and video representations. 
    \item We demonstrate that our approach can generalize to natural language queries despite not training with human-annotated captions. 
    \item We conduct extensive source sound separation experiments across 4 different datasets including SOLOS, MUSIC, UMRP and AudioSet, where we outperform state-of-the-art strongly-supervised approaches by a significant margin.
\end{enumerate}


==> old_introduction_v5.tex <==
\section{Introduction v5}

%\bryan{Our everyday audiovisual world is composed of many different visible objects making sounds, often with multiple sources sounding simultaneously. For example, consider the video of the guitar and cello musicians playing together in Figure 1. The depicted cello and guitar have distinct timbres, and the musicians play non-unison, but complementary melodies. We seek to allow a user to select a sounding object given a natural language query, such as ``person playing a guitar'', and for a system to automatically separate the sound source from the input audio waveform and to localize the sound source in the input video. Achieving this goal would enable important downstream applications including holistic video understanding [], embodied AI [], and bidirectional audio-to-video retrieval [].}

%Moreover, the visual appearance and motion of the objects give clues about the different sources' sounds. An important problem (known as {\em sound source separation}) is to separate the different sound sources given a sound mixture.

%Traditionally, this task is formulated without knowledge of the sound sources' names []. Natural language provides an intuitive and flexible interface for selecting the different sound sources. For example, an ideal system could take the natural language query ``person playing a guitar'' and return the separated guitar sound.

\ks{Mention the weakness of prior work here, ie supervision. "Bad guy" first, then "hero"!}
Recent vision-and-language pretraining approaches [] have focused on learning strong transferable visual and text representations from web-scale image and text collections, that can generalize to downstream tasks with little to no finetuning on the target datasets. Their success has demonstrated the much higher quality \ks{strength?} of supervision present in noisy large-scale corpuses sourced from the web as compared to smaller and human-annotated datasets. Since natural language has the generality to express a large and varied range of visual concepts, it provides an intuitive and flexible interface for separating sounds in a mixed audio. To this end, we aim to learn to separate audio source components in videos based on natural language queries without any supervision. This is motivated by our observation that the co-occurrence of a sounding object and its depiction in a video provides useful cues for helping a model learn to identify and separate the sound from the background. Consequently, we seek to learn these co-occurrences from unlabeled audio-video pairs.

By itself, separating audio sources in videos or based on natural language queries is already an inherently difficult problem since the input audio is usually a mixture of sounds from different objects and there is a lack of ground-truth source annotations. This is greatly compounded by our key challenge of how to jointly localize sounding objects in both a video and an audio waveform as well as associate both with natural language in a completely self-supervised way. To ease the difficulty, \ks{Start 2nd par. with this:} state-of-the-art audio-visual separation approaches often rely on training object detectors [] with strong supervision using video labels and learning to associate separated audio sources with bounding boxes that are detected for a set of fixed-vocabulary categories (Figure~\ref{fig:latent_motiv} top). However, this may not always be feasible due to insufficient bounding box annotations for objects in the long-tailed distribution. More importantly, this severely curtails their flexibility to scale up training to a larger and more diverse set of visual concepts.

With this in mind, our objective is to address the above-mentioned limitations by learning to separate audio sources based on any combination \ks{what does 'any combination' mean?} of video and natural language queries without strong supervision, illustrated in Figure~\ref{fig:latent_motiv} (bottom). We believe that alleviating the need for human-annotated captions and bounding box supervision during training will open up the possibility for learning to perform multimodal audio source separation from the plethora of unlabeled videos online, allowing approaches to generalize well to a large variety of audio sources and visual concepts.
\uri{Maybe you can talk about how self-supervised approaches have lately surpassed models trained on strongly labeled datasets due to the differences in the amount of training data (e.g., cite CLIP and Whisper).}
Similar to how humans often leverage object sounds to understand their states and interactions with other objects, multimodal audio source separation is integral to improving machine perception of our environment. It has important implications in downstream applications including holistic video understanding [], embodied AI [] and bidirectional audio-to-video retrieval [].

We propose the first completely self-supervised approach for learning to separate audio source components with text and/or video queries from unlabeled videos without object labels or text captions at all \ks{well, technically CLIP is trained on text captions, maybe just say 'unlabeled videos'}. Our proposed \modelname approach uses a Multiple Instance Learning (MIL) formulation to learn to perform source separation at the \emph{region} level, without making assumptions on the presence of objects in the videos, by leveraging the recent success of vision-and-language foundation models [] (\eg CLIP and ALIGN) to overcome the above-mentioned challenges. The absence of text captions or object labels in these videos raises the question of how we can learn to separate audio components with natural language queries despite not training with them. To  this end, we adapt pretrained vision-and-language foundation models to extract latent concepts \ks{define this term} and leverage them for pseudo-target supervision in the form of two novel loss functions. \ks{the following is hard to understand, maybe just cut or replace with high level intuition} These loss formulations stem from our key intuition that a model has to learn a strong alignment between the visual, language and audio representations such that text and videos can be used interchangeably or in combination to perform source separation. We impose cyclic consistency losses where the spatiotemporal region features in the video are first used to separate the corresponding audio source before maximizing the similarity between the representation of the final predicted audio source and the latent concept in two different ways. Intuitively, this allows the model to identify regions with the most relevant visual concepts for source separation, facilitating its ability to learn from multi-source videos without prior knowledge of possible objects or their positions. \ks{what is the key novel idea here? just replace object detectors with CLIP? Or something more?}

Despite not relying on trained object detectors, our proposed approach outperforms strongly-supervised state-of-the art-approaches by a significant margin across multiple datasets. More significantly, we demonstrate that our trained model can also separate sound sources based on natural language queries despite not having access to ground-truth object labels or using text representations during training. In summary, our contributions are listed as follows:
\begin{enumerate}
    \item We propose the first fully self-supervised approach to learn to separate audio source components with video and/or natural language queries from unlabeled videos.
    \item We introduce two novel loss functions that leverage latent concepts to learn a strong alignment between the audio, text and video representations. 
    \item We demonstrate that our approach can generalize to natural language queries despite not training with human-annotated captions.\ks{our approach uses NL queries as input? so what does it mean to 'generalize' to them? Maybe say 'use'?} 
    \item We conduct extensive source sound separation experiments across 4 different datasets including SOLOS, MUSIC, UMRP and AudioSet, where we outperform state-of-the-art strongly-supervised approaches by a significant margin.\ks{this seems kind of too good to be true, I would at least mention the power of V&L pretraining for this, and how transferring that power to this problem gives us nice results, rather than keep saying we use no supervision at all.}
\end{enumerate}

